IBADR: an Iterative Bias-Aware Dataset Refinement Framework for Debiasing NLU models

As commonly-used methods for debiasing natural language understanding (NLU) models, dataset refinement approaches heavily rely on manual data analysis, and thus maybe unable to cover all the potential biased features. In this paper, we propose IBADR, an Iterative Bias-Aware Dataset Refinement framework, which debiases NLU models without predefining biased features. We maintain an iteratively expanded sample pool. Specifically, at each iteration, we first train a shallow model to quantify the bias degree of samples in the pool. Then, we pair each sample with a bias indicator representing its bias degree, and use these extended samples to train a sample generator. In this way, this generator can effectively learn the correspondence relationship between bias indicators and samples. Furthermore, we employ the generator to produce pseudo samples with fewer biased features by feeding specific bias indicators. Finally, we incorporate the generated pseudo samples into the pool. Experimental results and in-depth analyses on two NLU tasks show that IBADR not only significantly outperforms existing dataset refinement approaches, achieving SOTA, but also is compatible with model-centric methods.

==> table/intro_case.tex <==
\begin{table}[tb]
\small
\center
\renewcommand{\arraystretch}{1.1}
\begin{tabularx}{0.45\textwidth}{ l }
\toprule[1pt]
\makecell[l]{\textbf{Premise}:  \textit{The manager knew the tourists supported the author .} \\ 
\textbf{Hypothesis}:  \textit{The manager knew the tourists .} \\  
\textbf{Golden Label}:  \textit{contradiction} \\
\textbf{Predicted Label}:  \textit{\textcolor{red} {entailment}}} \\
\hline
\makecell[l]{\textbf{Premise}:  \textit{The student saw the managers .} \\ 
\textbf{Hypothesis}:  \textit{The managers saw the student .} \\ 
\textbf{Golden Label}:  \textit{contradiction} \\
\textbf{Predicted Label}: \textit{\textcolor{red}{entailment}}} \\
\bottomrule[1pt]
\end{tabularx}
\caption{Two instances from HANS \cite{McCoyPL19}. Both instances contain biased features, which make the dominant model \cite{devlin-etal-2019-bert} unable to accurately predict the relationship between the premise and hypothesis. In the first instance, the hypothesis is a sub-sequence of the premise, while they convey different meanings. In the second one, the premise and hypothesis share identical words, but with swapped objects.}
\label{tab:case_intro}
\end{table} 


==> table/mnli_rt.tex <==
\begin{table*}[!t]
\centering

\begin{tabular}{lccc}
\hline
\textbf{Method}                        & \textbf{MNLI dev-m} & \textbf{MNLI dev-mm} & \textbf{HANS}  \\ \hline
\multicolumn{4}{l}{\textit{\textbf{Prior model-centric methods}}}                  \\ \hline
PoE \cite{karimi-mahabadi-etal-2020-end}                           & 84.58      & 84.85       & 66.31 \\ \hline
Learned-Mixin \cite{clark-etal-2019-dont}                 & 80.50      & 81.20       & 64.00 \\ \hline
Conf-reg \cite{utama-etal-2020-towards}                      & 84.60      & 85.00       & 69.10 \\ \hline
\multicolumn{4}{l}{\textit{\textbf{Prior dataset refinement methods}}}             \\ \hline
z-filter (z-aug) \cite{wu2022generating}              & \textbf{84.72}      & \textbf{85.14}       & 62.57 \\ \hline
z-filter (par-z) \cite{wu2022generating}              & 82.48      & 82.95       & 65.11 \\ \hline
z-filter (seq-z) \cite{wu2022generating}              & 82.55      & 83.17       & 67.69 \\ \hline
\multicolumn{4}{l}{\textit{\textbf{Model trained on our augment dataset}}}          \\ \hline
IBADA (second indicator)       & 84.08      & 83.94       & \textbf{68.90} \\ \hline
IBADA (update shallow model)   & 83.89      & 84.03       & 68.34 \\ \hline
IBADA (second indicator) + PoE & 84.61      & 84.22       & \textbf{69.64} \\ \hline
\end{tabular}%
\caption{Accuracy on MNLI-matched (MNLI dev-m), MNLI-mismatched (MNLI dev-mm), and HANS. Our framework effectively balances the performance on both the dev set and the challenge set. Additionally, it exhibits promising results when combined with model-centric approaches such as POE, further enhancing overall performance.}
\label{tab:mnli results}
\end{table*}
